LDKP: A Dataset for Identifying Keyphrases from Long Scientific Documents

Identifying keyphrases (KPs) from text documents is a fundamental task in natural language processing and information retrieval. Vast majority of the benchmark datasets for this task are from the scientific domain containing only the document title and abstract information. This limits keyphrase extraction (KPE) and keyphrase generation (KPG) algorithms to identify keyphrases from human-written summaries that are often very short (approx 8 sentences). This presents three challenges for real-world applications: human-written summaries are unavailable for most documents, the documents are almost always long, and a high percentage of KPs are directly found beyond the limited context of title and abstract. Therefore, we release two extensive corpora mapping KPs of ~1.3M and ~100K scientific articles with their fully extracted text and additional metadata including publication venue, year, author, field of study, and citations for facilitating research on this real-world problem.

==> candidate_kp_table.tex <==
\begin{table}[]
\begin{tabular}{lrr}
\hline
\textbf{Algorithm} & \multicolumn{1}{l}{\textbf{LDKP3K}} & \multicolumn{1}{l}{\textbf{LDKP10K}} \\ \hline
\textbf{SGRank}          & 86.96                      & 85.56                       \\ \hline
\textbf{TopicRank}       & 636.02                     & 520.81                      \\ \hline
\textbf{PositionRank}    & 678.65                     & 547.66                      \\ \hline
\textbf{TopicalPageRank} & 709.51                     & 574.50                      \\ \hline
\textbf{Singlerank}      & 773.11                     & 624.25                      \\ \hline
\textbf{TextRank}        & 773.11                     & 624.25                      \\ \hline
\textbf{Multipartite}    & 636.02                     & 520.78                      \\ \hline
\textbf{Yake}            & 2475.20                    & 1965.73                     \\ \hline
\textbf{TfIDF}           & 6472.93                    & 4922.29                     \\ \hline
\textbf{KPMiner}         & 79.51                      & 74.81                       \\ \hline
\textbf{WINGNUS}         & 659.47                     & 544.91                      \\ \hline
\textbf{Kea}             & 2534.71                    & 2032.84                     \\ \hline

\end{tabular}
\caption{Average number of candidate keyphrases generated by the ranking algorithms on LDKP3K and LDKP10K datasets.}
\label{tab:avg_num_candidates}
\end{table}

==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}

In this section, we describe our methodology to evaluate several popular keyphrase extraction algorithms on the proposed \textsc{LDKP3k} and \textsc{LDKP10k} datasets. We further report the benchmark results and also discuss the comparative advantage of different algorithms to provide future research direction.  
\subsection{Unsupervised Methods}
There are multiple unsupervised methods for extracting keyphrases from a document. We used the following popular graph-based algorithms: TextRank \cite{mihalcea-tarau-2004-textrank}, PositionRank \cite{florescu-caragea-2017-positionrank}, SingleRank \cite{singlerank}, TopicRank \cite{bougouin-etal-2013-topicrank}, and SGRank \cite{danesh-etal-2015-sgrank}. These algorithms first identify the candidate keyphrases using lexical rules followed by ranking the candidates using a graph-based approach.
% We tuned the parameters of our unsupervised algorithms on training dataset and then the testing was done on the test set using these best parameters.

\label{table:candidate_kp}
\input{candidate_kp_table}

\begin{table*}[htbp]
\scalebox{.87}{
\begin{tabular}{c|cc|cc|cc|cc|cc}
\hline
\multirow{2}{*}{\textbf{Method}} &
  \multicolumn{2}{c|}{\textbf{Krapivin}} &
  \multicolumn{2}{c|}{\textbf{NUS}} &
  \multicolumn{2}{c|}{\textbf{SemEval-2010}} &
  \multicolumn{2}{c|}{\textbf{LDKP3k}} &
  \multicolumn{2}{|c}{\textbf{LDKP10k}} \\ \cline{2-11} 
 &
  \textbf{F1@5} &
  \textbf{F1@10} &
  \textbf{F1@5} &
  \textbf{F1@10} &
  \textbf{F1@5} &
  \textbf{F1@10} &
  \textbf{F1@5} &
  \textbf{F1@10} &
  \textbf{F1@5} &
  \textbf{F1@10}\\ \hline
\textbf{PositionRank} &
  0.042 &
  0.052 &
  0.060 &
  0.086 &
  0.074 &
  0.098 &
  0.059 &
  0.062 &
  0.052 &
  0.061 \\ \hline
\textbf{TextRank} &
  0.036 &
  0.047 &
  0.071 &
  0.090 &
  0.085 &
  0.117 &
  0.082 &
  0.094 &
  0.068 &
  0.074 \\ \hline
\textbf{TopicRank} &
  0.071 &
  0.080 &
  0.130 &
  0.152 &
  0.111 &
  0.132 &
  0.108 &
  0.110 &
  0.098 &
  0.102 \\ \hline
\textbf{SingleRank} &
  0.001 &
  0.003 &
  0.005 &
  0.008 &
  0.009 &
  0.010 &
  0.016 &
  0.025 &
  0.011 &
  0.014 \\ \hline
\textbf{MultipartiteRank} &
  0.103 &
  0.107 &
  0.150 &
  0.193 &
  0.116 &
  0.145 &
  0.129 &
  0.110 &
  0.104	&
  0.106 \\ \hline
\textbf{TopicalPageRank} &
  0.009 &
  0.012 &
  0.046 &
  0.059 &
  0.014 &
  0.024 &
  0.019 &
  0.027 &
  0.020 &
  0.031 \\ \hline
  
\textbf{SGRank} &
  0.140 &
  0.131 &
  0.195 &
  0.203 &
  0.177 &
  0.201 &
  0.138 &
  0.128 &
  0.136 &
  0.132 \\ \hline
  \end{tabular}
  }
%\vspace{-2 mm}
\caption{Results on long document datasets using unsupervised graph-based models}
\label{tab:results}
\end{table*}

\begin{table*}[htbp]
\scalebox{.87}{
\begin{tabular}{c|cc|cc|cc|cc|cc}
\hline
\multirow{2}{*}{\textbf{Method}} &
  \multicolumn{2}{c|}{\textbf{Krapivin}} &
  \multicolumn{2}{c|}{\textbf{NUS}} &
  \multicolumn{2}{c|}{\textbf{SemEval-2010}} &
  \multicolumn{2}{c|}{\textbf{LDKP3k}} &
  \multicolumn{2}{|c}{\textbf{LDKP10k}} \\ \cline{2-11} 
 &
  \textbf{F1@5} &
  \textbf{F1@10} &
  \textbf{F1@5} &
  \textbf{F1@10} &
  \textbf{F1@5} &
  \textbf{F1@10} &
  \textbf{F1@5} &
  \textbf{F1@10} &
  \textbf{F1@5} &
  \textbf{F1@10}\\ \hline
  
  \textbf{TFIDF} &
  0.033 &
  0.052 &
  0.063 &
  0.111 &
  0.062 &
  0.070 &
  0.093 &
  0.099 &
  0.072 &
  0.080 \\ \hline

\textbf{KPMiner} &
  0.125 &
  0.151 &
  0.169 &
  0.212 &
  0.155 &
  0.181 &
  0.164 &
  0.152 &
  0.151 &
  0.142 \\ \hline

\textbf{Yake} &
  0.105 &
  0.107 &
  0.177 &
  0.235 &
  0.088 &
  0.129 &
  0.140 &
  0.132 &
  0.114 &
  0.114 \\ \hline

  \end{tabular}
  }
%\vspace{-2 mm}
\caption{{Results on long document datasets using unsupervised statistical models.}}
\label{tab:results}
\end{table*}

\subsection{Supervised Methods}
For supervised keyphrase extraction, we marked all the words in the document belonging to keyphrases as `B' or `I' depending on whether they are the first word of keyphrase or otherwise. Every other word, i.e. which was not part of any keyphrase got tagged as `O'. Then the keyphrase extraction task is posed as a supervised sequence tagging problem to predict `B', `I', and `O' labels.

Note that most supervised models like BERT \cite{bert} can accommodate text only up to 512 tokens long. To extract keyphrase from long documents, however we need models which can accommodate long texts. On the other hand, recently introduced models Longformer \cite{longformer}, Bigbird \cite{big_bird}, and Reformer \cite{Reformer} are specifically designed to handle longer pieces of text. In our experiments, we used LongFormer mainly due to its memory efficient implementation, thus making it an excellent choice for processing long documents. Unfortunately, in spite of being extremely powerful, Longformer can accommodate only up to 4098 tokens due to its design constraints. To work around this, we used the important sections like Title, Abstract, Introduction, Conclusion, Discussion, Results, and Related Work, as the input since they contained most of the keyphrases. Following \cite{longformer} Longformer was initialized with \textit{Longformer Base} model and trained using Cross-entropy loss using batch size of 2 for four full passes over the entire corpus using a single RTX 3090 GPU. 
% However, we observed that apart from Longformer most of these models are severely memory-inefficient and hard to train on a practical dataset. 

% However, we were able to train Longformer only due to resource constraints and as other models were not much GPU friendly. Longformer can accommodate up to 4098 token lengths and uses windows attention and global attention by customizing CUDA kernels. We trained Longformer on token classification task to provide the community with a baseline on Keyphrase extraction from Long documents.

% \subsection{Data Preprocessing}
% Our dataset has been converted to CoNLL-2003 format. %We identified the location of keyphrases in the text. 
% All the words in the document belonging to keyphrase were tagged as 'B' or 'I' depending on whether they are the first word of keyphrase or otherwise. Other words which were not part of any keyphrase were tagged as 'O'. Since Longformer could accommodate up to 4098 tokens, we used only important sections like Title, Abstract, Introduction, Conclusion, Discussion, Results, and Related Work, as statistically, they contained most of the keyphrases as shown in Figure-\ref{fig:analysis}(a).
% We initialized Longformer layer with pretrained \textit{Longformer Base} model as specified in \cite{longformer} paper and classification layer with a random weight. We then fine-tuned it on the token classification task to predict 'B', 'I', and 'O' labels. We used Cross-entropy as a loss function. We trained it till we got stable results on evaluation for test split of the dataset. It took around four epochs with a batch size of 2 on a single RTX 3090 GPU for most of the scenario.  

  
  
\begin{table*}[]
\scalebox{.87}{
\begin{tabular}{c|cc|cc|cc|cc|cc}
\hline
\multirow{2}{*}{\textbf{Method}} &
  \multicolumn{2}{c|}{\textbf{Krapivin}} &
  \multicolumn{2}{c|}{\textbf{NUS}} &
  \multicolumn{2}{c|}{\textbf{SemEval-2010}} &
  \multicolumn{2}{c|}{\textbf{LDKP3k}} &
  \multicolumn{2}{|c}{\textbf{LDKP10k}} \\ \cline{2-11} 
 &
  \textbf{F1@5} &
  \textbf{F1@10} &
  \textbf{F1@5} &
  \textbf{F1@10} &
  \textbf{F1@5} &
  \textbf{F1@10} &
  \textbf{F1@5} &
  \textbf{F1@10} &
  \textbf{F1@5} &
  \textbf{F1@10}\\ \hline

\textbf{Kea} &
  0.041 &
  0.063 &
  0.069 &
  0.134 &
  0.077 &
  0.090 &
  0.109 &
  0.118 &
  0.087 &
  0.096 \\ \hline

\textbf{WINGNUS} &
  0.059 &
  0.151 &
  0.057 &
  0.085 &
  0.059 &
  0.152 &
  0.099 &
  0.109 &
  0.093 &
  0.102 \\ \hline

\textbf{Bert} &
  0.265 &
  0.267 &
  0.307 &
  0.339 &
  0.162 &
  0.171 &
    0.358 &
    0.361 &
    0.240 &
    0.243 
 \\ \hline
  
\textbf{Longformer(4096 tokens)} &
  0.229 &
  0.232 &
  0.253 &
  0.284 &
  0.203 &
  0.219 &
  0.317 &
  0.319 &
  0.309 &
  0.340 \\ \hline
  
 \textbf{Longformer(512 tokens)} &
  - &
  - &
  - &
  - &
  - &
  - &
    0.257 &
    0.262  &
    0.246 &
    0.252 
 \\ \hline
 
\end{tabular}
}

%\vspace{-2 mm}
\caption{{Results on Long document datasets on Supervised models}}
\label{tab:results}
\end{table*}

\begin{table}[]
\adjustbox{width=\columnwidth}{
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Model} & \textbf{Dataset} & \textbf{Ground truth used} & \multicolumn{1}{l|}{\textbf{F1@5}} & \multicolumn{1}{l|}{\textbf{F1@10}} \\ \hline
Longformer & LDKP3k & Longformer & 0.358309 & 0.362957 \\ \hline
Bert & LDKP3k & Bert & 0.357925 & 0.360629 \\ \hline
Bert & LDKP3k & Longformer & 0.328236 & 0.331269 \\ \hline \hline
Longformer & LDKP10k & Longformer & 0.326409 & 0.343332 \\ \hline
Bert & LDKP10k & Bert & 0.239801 & 0.242627 \\ \hline
Bert & LDKP10k & Longformer & 0.196547 & 0.20044 \\ \hline
\end{tabular}%
}
\caption{{Comparison of Bert & Longformer performance}}
\label{tab:comparison}
\end{table}
\subsection{Evaluation Metrics}
% The evaluation metrics that we have used for evaluating our dataset are precision, recall and F1 scores. Here \textbf{Precision} is defined as the number of correctly matched keyphrases divided by the total number of predicted keyphrases. \textbf{Recall} is number of correctly matched keyphrases divided by the number of ground truth keyphrases. The \textbf{F1-score} is the harmonic mean of these two terms. The matched keyphrases refers to the keyphrases present in both predicted and ground truth keyphrases after stemming them.
We have used macro-averaged $F1@5$ and $F1@10$ as our evaluation metrics. Before evaluating, we lower-cased, stemmed, and removed punctuation from ground truth and predicted keyphrases. \\
Let $Y$ denote the ground truth keyphrases and $\bar{Y} = (\bar{y_1},\bar{y_2}, \dots, \bar{y_m})$ denote the predicted keyphrases ordered by their quality of prediction. Then we can define the metrics as follows:
\[
Precision@k = \frac{|Y \cap \bar{Y_k} |}{min\{\bar{|Y_k|},k\}}
\]
\[
Recall@k = \frac{|Y \cap \bar{Y_k} |}{|Y|}
\]
\[
F1@k = \frac{2*Precision@k*Recall@k}{Precision@k + Recall@k}
\]
where $\bar{Y_k}$ denotes the top k elements of the set $\bar{Y}$. 
% \textbf{add general defination of F1@k}

\subsection{Results}
We used the same baseline results as specified in \cite{rui_meng} for comparison between models trained on abstract and title only v/s our model trained on full documents. To make a fair comparison, we also used the same dataset split of NUS, Krapivin, and SemEval-2010 to train our supervised and unsupervised model. The only difference is that instead of using abstract and title only, we used full document.

As expected, unsupervised algorithms like TextRank, PositionRank, and SingleRank did not perform well on long documents than short documents. One possible reason could be that unsupervised models learned more noise than learning context from long documents. On further analysis, we observed that SGrank outperforms every other algorithm if we consider F1@10 scores. While training the Textrank model, we observed that as the window size increases, the F1 scores improved, but the number of predicted keyphrases decreased. Due to this reason, the line graph of TextRank does not dip like other algorithms. The F1 scores between F1@1 to F1@30 for the \textsc{LDkp3k} testing dataset are given in Figure \ref{fig:unsup_res_kp20k}. A similar pattern was observed for the \textsc{LDkp10k} test dataset.

We used supervised algorithm Maui\cite{maui} and KEA\cite{KEA} for baseline and comparison with our Longformer model. As stated in Table \ref{tab:results}, Longformer outperformed almost all the baseline on NUS, Krapivin, and SemEval-2010 datasets. 
We used the medium train split for \textsc{LDkp3k} and \textsc{LDkp10k} to train Longformer token classification model. Longformer on \textsc{LDkp3k} (inspired from KP20k) is performing better than all of the baseline (i.e. Maui, KEA) and CopyRNN model in \cite{rui_meng} paper. Since the \textsc{LDkp3k} test dataset is a subset of the KP20k test dataset, it will not be fair to compare them.
We did not compare long document keyphrase extraction on the \textsc{LDkp10k} dataset as there is no previous reported score, and a generic split of the OAGKX dataset that is available.

==> interpretability.tex <==
\section{Interpretability}
\label{sec:interpretability}

Next, to understand the challenges associated with the long document keyphrase extraction task and how the two supervised algorithms (BERT and Longformer) are learning the task, we do an interpretability study over them. We use Integrated Gradients (IGs) \cite{sundararajan2017axiomatic} for attributing the BIO tags to words, phrases and sections.  \\

\textbf{Setup}
The interpretability experiments/statistics were conducted over 1500 Integrated Gradients attribution maps for BERT and Longformer which were created using the accurate KeyPhrase predictions for 100 samples. The Figures~\ref{figure:attn_patterns} and~\ref{figure:comb_attn_patterns} show these attribution plots, where \textcolor{red}{red} shading denotes negative attribution, and \textcolor{green}{green} shading denotes positive attribution. \\

\textbf{Effect of Length:} 
Document length has two effects: one, additional keyphrases are found in the longer document length and two, the additional context length helps in better extraction of keyphrases. We evaluate the effect of length on both these counts using our interpretability experiments. 

\begin{figure}[htp]
    \includegraphics[width=8cm]{acl-ijcnlp2021-templates/ig_plots/kp_cdf_set(1).pdf}
    \caption{CDF of Avg. Key-phrase count (first occurrence counted) in buckets of 20 words}
    \label{figure:kpe_countvslength_cdf}
\end{figure}

\begin{figure}[htp]
   \includegraphics[width=8cm]{acl-ijcnlp2021-templates/ig_plots/cho_new(1).pdf}\vspace{1mm} \hline \vspace{1mm}
    \includegraphics[width=8cm]{acl-ijcnlp2021-templates/ig_plots/quet_new(1).pdf}\vspace{1mm} \hline \vspace{1mm}
    \includegraphics[width=8cm]{acl-ijcnlp2021-templates/ig_plots/integral_new(1).pdf}
    \caption{Integrated Gradients attribution maps for Keywords Cho, Quet and Integral respectively}
    \label{figure:attn_patterns}
\end{figure}

Fig~\ref{figure:attn_patterns} shows the IG plots for `begin' and `inside' classes for longformer for the keyphrase `Cho-quet-integral'. From the figures, we can note that the other occurrences of the KP are shaded, indicating that keyphrases themselves are important for detecting other keyphrases.     \includegraphics[width=8cm]{acl-ijcnlp2021-templates/ig_plots/articles_importances(1).pdf})

We calculate that on average, keyphrases pull 6.84 times the attribution weight compared to non-keyphrase words.
One key challenge faced by traditional datasets is that the region near the abstract (most KPE datasets) misses out on many keyphrases present in the heavy-tail of the KPE distribution within a document. This is shown by (Figure~\ref{figure:kpe_countvslength_cdf}), where only ~60\% of KPs are present in the first 200 tokens(included in the abstract). \\
Additionally, Fig.~\ref{figure:comb_attn_patterns} shows the average attribution values over all the keyphrase predictions. We can see that longformer has a number of peaks in the document end where the context length of BERT is not even able to reach. 
We posit that this helps longformer in achieving better results than BERT. Training longformer on a context size equal to BERT confirms this finding (Table~\ref{table:performance}).\\
Next we try to analyse the context size of BERT vs Longformer using aggregate statistics.
For longformer, the attribution values fall 63\% slower than BERT for 10-word intervals from the keyphrase location, words, thus indicating that longformer's gradients are more spread out than BERT. \\
We also calculate the ratio of attribution weights in the first 512 tokens of longformer to the next 3586 words (4098-512 words). It is spread in the average ratio of 14.38 in the first 512 tokens to the next 3586 words. Therefore, while the words near keyphrases are more important, there is a heavy-tail distribution which spreads till the end of the context length.
Fig.~\ref{figure:attvslength} demonstrates these stats by plotting how the attribution weights fall with sequence length for the single keyword prediction "Integral".\\ 
Table~\ref{table:attvslen} gives average sequence length for observing words in the top 90, 95, and 99 percentile attribution weights. We can note that longformer has, on average, 35\% higher sequence lengths for top-k percentile weighted words. 
It is important to note that all the sequence lengths in the Table~\ref{table:attvslen} are lower than the attention window of BERT and longformer. \\
In conclusion, longformer relies on a greater sequence length than BERT for identifying keyphrases, which likely boosts its performance. \\

\textbf{Effect of Linguistic Factors:}
Next we investigate some linguistic reasons for longformer's performance.
Due to scholarly nature of the corpus, we find that keyphrases have a high representation from academic words\footnote{We use the work by \citet{coxhead2000new} for the list of academic words} \cite{coxhead2000new}. We also see that academic words (words that appear frequently in academic text) are have 66.70\% higher attribution than nonacademic words. \\
Articles (`a', `an', `the') are considered as stop-words (unimportant words) in most NLP tasks and are often removed while processing text samples for those tasks. However, in keyphrase extraction, we note that articles carry a significant weight (Fig.~\ref{figure:articlesvslength}) and that articles around the intended keyphrase, on an average, have a higher weight than articles at other places. We find that this is the case since articles are used in conjunction with noun phrases and noun phrases have been shown to be useful for the task of keyphrase extraction \cite{nagy2011noun}.  \\
Therefore, we analyse the effect of longer document length, context length and linguistic preferences of longformer and how they affect its performance compared to BERT. \\

\begin{figure}[htp]
    \includegraphics[width=8.3cm]{acl-ijcnlp2021-templates/ig_plots/example2_combined_bert_attn.pdf}
    \vspace{0.01em}
    \hline 
    \vspace{1em}
    \includegraphics[width=8.3cm]{acl-ijcnlp2021-templates/ig_plots/example2_combined_long.pdf}
    \caption{Combined Integrated Gradients attribution patterns for Keywords of an article: Left - BERT, Right- LONGFORMER}
    \label{figure:comb_attn_patterns}
\end{figure}

% \begin{figure}[htp]
%     \includegraphics[width=8cm]{acl-ijcnlp2021-templates/ig_plots/kp_cdf_LIST.pdf}
%     \caption{CDF of Avg. Keyphrase count (all occurrences counted) in buckets of 200 words}
%     \label{figure:kpe_countvslength_cdf_list}
% \end{figure}

\begin{figure}[htp]
    \includegraphics[width=8.3cm]{acl-ijcnlp2021-templates/ig_plots/all_models_new(2).pdf}
    \includegraphics[width=8.3cm]{acl-ijcnlp2021-templates/ig_plots/all_models_new_integral_74(1).pdf}
    \caption{Comparing gradient weight maps for the 4096 length Longformer, 512 Longformer and BERT: Left- Averaged, Right- for a Keyword "INTEGRAL" at index 74}
    \label{figure:attvslength}
\end{figure}

\begin{figure}[htp]
    \includegraphics[width=8cm]{acl-ijcnlp2021-templates/ig_plots/articles_importances(1).pdf}
    \caption{Calculating the A, AN, THE attribution scores relative to their distance from keyphrase detected}
    \label{figure:articlesvslength}
\end{figure}

% Comparison of longformer-512 with BERT: By experimenting with different sizes of attention window for longformer, we also look at the effect of context length variation on long document keyphrase extraction.

% \textbf{Error Analysis:} 
% > Lower context length => Lower performance (proven by the facts that both longformer and bert lose some performance when trained on lower size of the attention window)
% > Lesser number of 

\begin{table}
{\begin{tabular}{|l||l||l|}
\hline
\textbf{Model} & \textbf{\makecell{Percentile\\Attention}} & \textbf{\makecell{Length from\\KP (NTokens)}} \\ \hline
  
BERT & 90 & 364.02\\ \hline
BERT & 95 & 322.27\\ \hline
BERT & 99 & 219.54 \\ \hline

LONGFORMER & 90 & 505.59\\ \hline
LONGFORMER & 95 & 429.23\\ \hline
LONGFORMER & 99 & 285.887 \\ \hline

\end{tabular}}
\caption{\label{table:attvslen}
\small
Comparing Attention vs Length for Bert AND Longformer 
}
\end{table}


\begin{table}
\scalebox{0.8}{
{\begin{tabular}{|l||l||l|}
\hline
\textbf{Model} & \textbf{\makecell{F1 Score}} & \textbf{\makecell{Accuracy Score}} \\ \hline

Longformer(512 tokens) & 25.33 & 96.8 \\ \hline
Longformer(4096 tokens) & 33.9 & 98.8 \\ \hline

\end{tabular}}}
\caption{\label{table:performance}
\small
Comparing Longformer Validation Performance for length 512 and 4096 
}
\end{table}

% bert has a lower context length + lesser no of keyphrases detected


% PERFORMANCE ON VALIDATION
% bert:{'test_loss': 0.1515083611011505, 'test_overall_precision': 0.36898923199167055, 'test_overall_recall': 0.2810954100482164, 
% 'test_overall_f1': 0.3191005378764543, 'test_overall_accuracy': 0.969
% longformer: {'test_loss': 0.16209611296653748, 'test_overall_precision': 0.4634380140082568, 'test_overall_recall': 0.26757356779431835, 
% 'test_overall_f1': 0.3392662057526534, 'test_overall_accuracy': 0.988
% longormer-trained 512: 'test_loss': 0.10273870825767517, 'test_overall_precision': 0.3382565987067595, 'test_overall_recall': 0.20245749090601473, 
% 'test_overall_f1': 0.2533042270291725, 'test_overall_accuracy': 0.968

==> semi-supervised.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Model} & \textbf{\#tokens} & \textbf{Sliding window} & \textbf{F1@5} & \textbf{F1@10} & \textbf{avg \#candidates} \\ \hline
bert           & 512               & 512                     & 21.4          & 20.5           & 22.5                      \\ \hline
longformer     & 512               & 512                     & 29.2          & 29.2           & 12.2                      \\ \hline
\end{tabular}
\end{table}
